ABot-PhysWorld: Interactive World Foundation Model for Robotic Manipulation with Physics Alignment

Video-based world models offer a powerful paradigm for embodied simulation and planning, yet state-of-the-art models often generate physically implausible manipulations - such as object penetration and anti-gravity motion - due to training on generic visual data and likelihood-based objectives that ignore physical laws. We present ABot-PhysWorld, a 14B Diffusion Transformer model that generates visually realistic, physically plausible, and action-controllable videos. Built on a curated dataset of three million manipulation clips with physics-aware annotation, it uses a novel DPO-based post-training framework with decoupled discriminators to suppress unphysical behaviors while preserving visual quality. A parallel context block enables precise spatial action injection for cross-embodiment control. To better evaluate generalization, we introduce EZSbench, the first training-independent embodied zero-shot benchmark combining real and synthetic unseen robot-task-scene combinations. It employs a decoupled protocol to separately assess physical realism and action alignment. ABot-PhysWorld achieves new state-of-the-art performance on PBench and EZSbench, surpassing Veo 3.1 and Sora v2 Pro in physical plausibility and trajectory consistency. We will release EZSbench to promote standardized evaluation in embodied video generation.

==> workshop/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> workshop/sec/0_abstract.tex <==
% \begin{abstract}
% Video generation has emerged as a compelling paradigm for building embodied world models, yet existing methods remain biased toward visual aesthetics at the expense of physical fidelity: generated videos frequently exhibit object penetration, gravity anomalies, and contact distortion. Meanwhile, injecting low-dimensional action commands into high-dimensional visual backbones through full fine-tuning causes catastrophic forgetting of pre-trained physical priors, and the field still lacks rigorous benchmarks for evaluating zero-shot physical consistency. We present a physically grounded, action-controllable embodied world model built on a 14-billion-parameter Diffusion Transformer, trained on a curated embodied video corpus with hierarchical distribution balancing across robot morphologies, tasks, and scenes. To enforce physical law compliance, we introduce an automated preference alignment pipeline in which a decoupled vision-language discriminator decomposes physics evaluation into proposing and scoring, and a memory-efficient Diffusion-DPO algorithm steers generation toward physically plausible predictions. For action-conditioned control, a parallel context-block mechanism converts robotic commands into spatial action maps and residually injects them via zero-initialized convolutions, enabling cross-embodiment generalization without eroding foundational priors. We further propose the Embodied-ZeroShot Benchmark (EZSbench) with compositionally synthesized out-of-distribution scenarios and a decoupled dual-model evaluation protocol. Our model establishes state-of-the-art physical fidelity, achieving Domain Scores of 0.9306 on PBench and 0.8366 on EZSbench, surpassing Veo~3.1 and Sora~v2~Pro by 11.4\% and 22.0\% respectively, while attaining the highest trajectory consistency in action-conditioned generation.
% \end{abstract}

% \begin{abstract}
% Current video generation models produce visually compelling outputs but routinely violate the physics of robotic manipulation: grippers pass through objects, rigid bodies deform on contact, and items move without applied force. This visual-physical gap persists because standard maximum-likelihood training treats physically correct and physically impossible predictions identically, providing no signal to penalize contact-level violations. We present ABot-PhysWorld, a 14B-parameter Diffusion Transformer that closes this gap through three mechanisms: (1)~supervised fine-tuning on three million manipulation clips curated with hierarchical distribution balancing and physics-aware captions, (2)~Diffusion-DPO post-training guided by a decoupled VLM discriminator that generates task-specific physical checklists, and (3)~a parallel context-block injection that converts action commands into spatial maps for cross-embodiment control without eroding the backbone's learned physics. On PAI-Bench, ABot-PhysWorld reaches a Domain Score of 0.9306, outperforming Veo~3.1 and Sora~v2~Pro by 11.4\% and 22.0\%, with the highest trajectory consistency in action-conditioned generation. We also release the Embodied-ZeroShot Benchmark (EZSbench) for out-of-distribution evaluation, where our model scores 0.8366, indicating that the physical alignment transfers to unseen robot-task-scene combinations.
% \end{abstract}

\begin{abstract}
Video-based world models offer a powerful paradigm for embodied simulation and planning, yet state-of-the-art models often generate physically implausible manipulations—such as object penetration and anti-gravity motion—due to training on generic visual data and likelihood-based objectives that ignore physical laws.
We present \textbf{ABot-PhysWorld}, a 14B Diffusion Transformer model that generates visually realistic, physically plausible, and action-controllable videos. Built on a curated dataset of three million manipulation clips with physics-aware annotation, it uses a novel DPO-based post-training framework with decoupled discriminators to suppress unphysical behaviors while preserving visual quality. A parallel context block enables precise spatial action injection for cross-embodiment control.
To better evaluate generalization, we introduce \textbf{EZSbench}, the first training-independent embodied zero-shot benchmark combining real and synthetic unseen robot-task-scene combinations. It employs a decoupled protocol to separately assess physical realism and action alignment.
ABot-PhysWorld achieves new state-of-the-art performance on PBench and EZSbench, surpassing Veo~3.1 and Sora~v2~Pro in physical plausibility and trajectory consistency. We will release EZSbench to promote standardized evaluation in embodied video generation.
\end{abstract}


